NeoMem: Hardware/Software Co-Design for CXL-Native Memory Tiering

The Compute Express Link (CXL) interconnect makes it feasible to integrate diverse types of memory into servers via its byte-addressable SerDes links. Considering the various access latency, harnessing the full potential of CXL-based heterogeneous memory systems requires efficient memory tiering. However, prior work can hardly make a fundamental progress owing to low-resolution and high-overhead memory access profiling techniques. To address this critical challenge, we propose a novel memory tiering solution called NeoMem, which features a hardware/software co-design. NeoMem offloads memory profiling functions to CXL device-side controllers, integrating a dedicated hardware unit called NeoProf. NeoProf readily monitors memory accesses and provides the OS with crucial page hotness statistics and other useful system state information. On the OS kernel side, we design a revamped memory-tiering strategy, enabling accurate and timely hot page promotion based on NeoProf statistics. We implement NeoMem on a real FPGA-based CXL memory platform and Linux kernel v6.3. Comprehensive evaluations demonstrate that NeoMem achieves 32% to 67% geomean speedup over several existing memory tiering solutions.

==> algorithm/hp_detection.tex <==
\begin{algorithm}[t]
\def\mathbi#1{\textbf{\em #1}}
% \small
\footnotesize
\label{algo:migration}
\caption{Hot Page Detection Algorithm}
\textbf{Input:} Page access stream $\mathbb{S}$; Threshold ${\theta}$; Hash functions $h_i(\cdot)$, $i\in[0,\mathbf{D}-1]$; Sketching array $A[\mathbf{D}][\mathbf{W}]$;  \\

\textbf{Output:} Hot page queue $HQ$; \\


$\triangleright$ Set $A[i][j].valid = False$, $i\in[0,\mathbf{D}-1], j\in[0,\mathbf{W}-1]$; \\
$\triangleright$ {Detect hot pages:} \\
Offset\_buffer $OB[\mathbf{D}]$ = \{0\}; \\

\While {$P$ = $S.get()$ } {  
$\textit{isNewHot} = \textit{False}$;  \textcolor{blue}{/*Used for new hot page detection*/} \\
$minCnt = MAX$; \\
\For{$i \leftarrow 0$ until $\mathbf{D}$} { 
 $j = h_i(P); OB[i] = j; $ \textcolor{blue}{/*Calculate and buffer hashed offset*/} \\ 
\If{$A[i][j].valid$}{
    $A[i][j]$.counter +=1;  \textcolor{blue}{/*Counter increment*/} \\
    $minCnt = min(minCnt, A[i][j].counter);$\\}
\Else{$A[i][j].counter = 1$; \\ $A[i][j].valid = \textit{True}$; \textcolor{blue}{/*New entry*/}}
}
\If{$minCnt > \theta$}{  
\For{$i \leftarrow 0$ until $\mathbf{D}$} { 
    
    $\textit{isNewHot} = isNewHot~\textbf{|}~ \sim A[i][OB[i]].hot;$ \textcolor{blue}\\  
    $A[i][OB[i]].hot = \textit{True}$ \textcolor{blue}{/*Set the hot bit */}}
    }
\If {$\textit{isNewHot}$}{$HQ.Enqueue(P)$; \textcolor{blue}{/*Record a new hot page*/}}
}
\textbf{Return} $HQ$;
\end{algorithm}



==> fig_tex/damon_overhead.tex <==
\begin{figure} [t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/resolution_compare.pdf} 
    \caption{Damon Overhead Comparison.}
    % \vspace{-1em}
         \label{fig:damon_overhead}
\end{figure}



==> fig_tex/page_tracking_cmp.tex <==
\begin{figure} [h]
    \centering
    \includegraphics[width=0.80\linewidth]{fig/page_tracking_cmp.pdf} 
    \caption{The obserbility gap. \todo{plot some real numbers}}
    % \vspace{-1em}
         \label{fig:page_tracking}
\end{figure}



==> fig_tex/pebs_overhead.tex <==
\begin{figure} [t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/pebs_overhead.pdf} 
    \caption{PEBS Overhead Comparison.}
         \label{fig:pebs_overhead_cmp}
\end{figure}



==> fig_tex/sketch_config.tex <==
\begin{figure} [t]
    \centering
    \includegraphics[width=1.0\linewidth]{fig/sketch_config.pdf} 
    % \vspace{-1em}
    \caption{Performance with Different Sketch Width ($\mathbf{W}$).}
    % \vspace{-1.5em}
         \label{fig:sketch_config}
\end{figure}



==> fig_tex/tlb_vs_llc.tex <==
\begin{figure} [t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/tlb_vs_llc.pdf} 
    \caption{In-accuracy of TLB-base Profiling.}
    % \vspace{-1em}
         \label{fig:tlb_vs_llc}
\end{figure}



==> fig_tex/tracking_tech_compare.tex <==
\begin{figure} [t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/page_tracking_comparison.pdf} 
    \caption{Comparison Among Page Tracking Mechanisms. LO: Low Overhead. TR: Time Resolution. SR: Space Resolution. GE: Generality. CA: Cache Awareness}
         \label{fig:page_tracking}
\end{figure}



==> table/benchmarks.tex <==
\begin{table}[t]
% \vspace{-1em}
% \centering
\caption{Benchmarking Applications}
\vspace{-0.5em}
\label{tab:benchmark}
\centering
\resizebox{0.495\textwidth}{!}{
\centering
\setlength{\tabcolsep}{1mm}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
Application & PR & XSBench & Silo & 603.bwaves & 654.roms & Btree & GUPS       \\ \midrule
RSS (GB)  & 17.5 & 17.1   & 15.3 &  11.1       &  10.3    & 19.7  & 19.6       \\ \bottomrule
\end{tabular}
}
}
\end{table}

==> table/memory_compare.tex <==
\begin{table}[t]
\caption{Latency and Bandwidth Estimation of Different Memory}

\resizebox{0.48\textwidth}{!}{\renewcommand{\arraystretch}{1.2}{
\begin{tabular}{|c|c|c|}
\hline
Memory Type        & R / W Latency (ns) & R / W BW (GB/s) \\ \hline
CPU-attached DRAM  & 81 / 82            & 120 / 82        \\ \hline
CXL-connected DRAM & 153 / 162          & 97 / 63         \\ \hline
CXL-connected PMem &                    &                 \\ \hline
\end{tabular}
}}
\end{table}

==> table/user_interface.tex <==
% \usepackage{multirow}
\begin{table}[t]
\caption{NeoProf user-space interface }
\label{tab:interface}
\centering
\resizebox{0.495\textwidth}{!}{
\centering
\begin{tabular}{|l|l|p{0.5\linewidth}|}
\hline
\multicolumn{1}{|c|}{\textbf{Parameter}} & \multicolumn{1}{c|}{\textbf{Type}} & \multicolumn{1}{c|}{\textbf{Description}} \\
\hline
\multirow{1}{*}{\texttt{neomem\_enabled}} & \multirow{1}{*}{Bool} & Enable NeoMem \\
\hline
\multirow{1}{*}{\texttt{hot\_threshold}} & \multirow{1}{*}{Int} & The threshold $\theta$ of hot pages. \\
\hline
\multirow{1}{*}{\texttt{migration\_interval}} & \multirow{1}{*}{Int ($\mu$s)} & Read out hot page information and migrate them. \\
\hline
\multirow{1}{*}{\texttt{clear\_interval}} & \multirow{1}{*}{Int} & Clear the states of NeoProf after a certain number of scanning rounds. \\
\hline
\multirow{1}{*}{\texttt{state\_sample\_interval}} & \multirow{1}{*}{Int} & Sample the read/write counts after every certain number of cycles. \\
\hline
\end{tabular}
}
\end{table}

==> tex/limitations.tex <==
% \section{Limitations}
% Current NeoMem prototype only equips a single 16GB CXL memory due to the hardware limitations. 



==> tex/response_letter.tex <==
\setcounter{page}{0}

\thispagestyle{empty}
\twocolumn[
\begin{@twocolumnfalse}
\section*{\centering{Cover Letter}}
\end{@twocolumnfalse}
]

\subsection{Summary of revision}

\noindent\textbf{\bone}. \emph{\textbf{Main contributions clarified.}} To clarify  our main contribution % , not the implementation of CXL IP 
 (\textbf{Review A/B}),
% or the entire memory-tiering system (Review \textbf{A}). 
we have revised the title and sections. Detailed introductions of Intel's CXL IP and its usage in NeoMem are added in Sec.\ref{sec:exp_setup} / \ref{sec:implementation}.  Fig-10 also adds a detailed block-diagram to showcase our proposed  parts.

\noindent\textbf{\btwo}. \emph{\textbf{Better explanation of the HW setup.}}  Fig.\ref{fig:bg_slowdown}-a has been better explained to understand the HW setup (\textbf{Review C}). The longer FPGA latency is discussed in Sec.\ref{sec:discussion} (\textbf{Review B}). 


\noindent\textbf{\bthree}. \emph{\textbf{More experiments added.} }Sec.\ref{sec:analysis} / \ref{sec:main_results} now include 1) CPU overhead of NeoMem (\textbf{Review A}).  2) Slow-tier traffic (\textbf{Review B}).  3) experiments on DeathstarBench (\textbf{Review C}). 4) \# of promotions/demotions comparison  (\textbf{Review D})
 
\noindent\textbf{\bfour}. \emph{\textbf{More related work and descriptions.}} More related work in Sec.\ref{sec:related_work} (\textbf{Review A}/\textbf{D}). More in-depth descriptions of baseline methods in Sec.\ref{sec:memory_profiling} and  Sec.\ref{sec:exp_setup} (\textbf{Review E})


% \vspace{2pt}
\subsection{Responses to comments} 

\noindent\textbf{To review A:}

% \noindent$\bullet$   \emph{\textbf{Add the sketch usage in related work.}}

% Please see revision 3. 

\noindent$\bullet$ \emph{\textbf{More related usage of sketch? Why we chose sketch over other similar algorithms?}} Please refer to  Sec.\ref{sec:sketching_works}. 
% Hope that we could inspire the community to find better hot-page detectors for device-side profiling. 

\noindent$\bullet$ \emph{\textbf{The  scope  is a bit overstated.}} We've adjusted presentations to specify the scope,  such as changing ``NeoMem system" to ``NeoMem solution", etc. Please refer to revision point \bone.  

\noindent$\bullet$ \emph{\textbf{The CPU overhead?}} CPU overhead evaluated in Sec.\ref{sec:analysis}.  

% \vspace{0.5em}
\noindent\textbf{To review B:}

\noindent$\bullet$ \emph{\textbf{Misrepresentation of contributions and CXL implementation?}}
 We regret any confusion here, but we did not claim to have implemented a CXL IP. Our main contributions are the  NeoProf hardware  and NeoMem software.  We have clarified this and corrected some mistakes in describing intel's CXL IP implementation.  Please refer to revision point \bone.

% \noindent$\bullet$ \emph{\textbf{Overlook of CXL latency.}}
% Yes, in Fig.10-a it is not approperate to say that the green part is CXL IP. It is actually the R-tile (CXL chiplet) controller or interface.  Thank you for pointing it out and we have modified the notation in the revised version.   


\noindent$\bullet$ \emph{\textbf{Overlooked CXL latency?}}
Certainly, Intel's CXL FPGA implementation results in longer latency. However, NeoMem's efficacy persists even with a lower latency. Given that TPP targets 170-250ns latency and still yields 18\% performance improvement, NeoMem will perform better in such situations as it is substantially superior to TPP according to our evaluations. 
% Furthermore, the 430ns latency aligns with scenarios where slower memory medias are connected via CXL. 
We have revised Sec.~\ref{sec:discussion} to include more discussions.
% and add a new experiment to evaluate NeoMem's performance under differerent CXL latency \todo{in Sec.XXX}.
% Note that the 170-250ns latency from TPP and Pond stems from NUMA emulation, not an actual EP implementation.  The only EP implementation, DirectCXL~\cite{gouk2022direct}, also reports a 426ns CXL-memory latency (Table-2 in DirectCXL) even at a scaled-up frequency. 

% We agree that  Intel's CXL FPGA has not met the low latency expectations of the CXL community. 
% But it is worth noting that the only EP implementation by far, the DirectCXL~\cite{gouk2022direct} also reports 426ns of CXL-memory latency even when scaling the IP frequency to 1.2GHz (Table-2 in DirectCXL). 
% The 170-250ns latency reported by TPP and Pond is from NUMA emulation in a two-socket system, not from a real EP implementation. Despite this, NeoMem maintains its value even with an ideal 170ns CXL latency. This is because, firstly, TPP and Pond have shown that memory tiering is still necessary at this latency. Secondly, CXL's ability to connect slower memory medias like NVM to the host CPU, resulting in higher latency than CXL+DRAM, necessitates memory-tiering optimization (Fig.\ref{fig:cxl_mem}).
% TPP and Pond use two-socket NUMA system to simulate CXL so the 170-250ns latency is from NUMA emulation rather than testing from real EP implementation. We also would like to emphasize that NeoMem's value will not be diminished even with an ideal 170ns of CXL latency for two reasons: (1) TPP and Pond have proven that even with 170ns of latency, memory tiering is also necessary for performance improvement. (2) As also illustrated in Fig.\ref{fig:cxl_mem}, CXL enables seamlessly connecting slower memory medias such as NVM to the host CPU, their latency will be much higher than CXL+DRAM, which heavily relies on memory-tiering optimization.  
% The NUMA-based emulation is 
% In fact, a smaller CXL latency will not hurt the conclusion of this paper.    

\noindent$\bullet$ \emph{\textbf{The ASIC implementation lacks substance.}} Admittedly, this is not a complete ASIC implementation. Our purpose is to  estimate  the hardware overhead of NeoProf co-processor. To avoid any confusion, we've clarified this and  renamed this subsection in Sec.\ref{sec:discussion} as ``Hardware Overhead Estimation". 

\noindent$\bullet$ \emph{\textbf{Limitations due to CXL 1.1 specification?}} We would like to emphasize that NeoMem can also support multi-host CXL-3.0 via small modifications. Please refer to discussions in Sec.\ref{sec:discussion}.

\noindent$\bullet$ \emph{\textbf{Challenges in accelerating random workloads.}} NeoMem  leverages the pervasive data locality in  workloads~\cite{tpp,pond}. 
% Fortunately, most data-center workloads, as also evaluated by TPP and Pond, exhibit good data locality. 
For highly random workloads, NeoMem automatically moderates migration aggressiveness in response to increased ping-pong severity (Sec.\ref{sec:policy}), preventing performance decline.

\noindent$\bullet$ \emph{\textbf{Slow/fast memory accesses analysis.}}  Added in Sec.\ref{sec:analysis}.

\noindent$\bullet$ \emph{\textbf{Detailed explanation for some eval. results, e.g., Fig.12.}} More explanations added in Sec.\ref{sec:eval}. The slightly higher performance on the 1:4 configuration in Fig.\ref{fig:different_mem_configs} is  due to system noise. We will release the code to ensure reproducibility.


% In Fig.12, the slight performance improvement in the 1:4 configuration over the 1:2 configuration is entirely due to normal system fluctuations during the two experiments. Theoretically, the performance of the two should be similar since the hot set of GUPS can always fit into local DRAM, and a slight advantage for either is to be expected in  experiments. We have added more explanations in the evaluation section.  


% \vspace{2pt}
\noindent\textbf{To review C:}

% \noindent$\bullet$ \emph{\textbf{how more ``precise'' monitoring techniques are leveraged?}}

% As illustrated in Fig.~\ref{fig:motivation_converge}, NeoMem converges better than the other baselines and has less fluctuation. 

% \noindent$\bullet$ \emph{\textbf{Why is higher profiling frequency required?}}

% Low frequency profiling cannot efficiently detect hot pages. \todo{ref some paper?}

\noindent$\bullet$ \emph{\textbf{Why TPP reports low performance impact from hotness monitoring?}} TPP minimizes performance impact by substantially lowering profiling resolution (1-60s interval versus NeoMem's 10ms). However, as shown in Fig.\ref{fig:performance_overview} and Fig.\ref{fig:motivation_converge}, this reduced resolution may not suffice for many workloads.

% \noindent$\bullet$ \emph{\textbf{Hardware overhead of NeoMem?}} As discussed in Sec.~\ref{sec:discussion}, NeoMem introduces 5.3 $mm^2$ additional logic.



\noindent$\bullet$ \emph{\textbf{Experiments on  DeathstarBench?}} Added in Sec.\ref{sec:eval}.


\noindent$\bullet$ \emph{\textbf{Does NeoMem break up huge pages?}} In current experiments, transparent huge pages are disabled for simplicity. For future work enabling huge pages, NeoMem can break up huge pages into 4kB pages to achieve a higher spatial resolution. 

% \vspace{4pt}
\noindent\textbf{To review D:}

\noindent$\bullet$ \emph{\textbf{Why focus on CXL?}}
NeoMem could be adapted to other bus-extended systems like CCIX and GEN-Z. We focus on CXL  as it  has garnered significant support from the community and we can buy commercial products to perform experiments.    

\noindent$\bullet$ \emph{\textbf{Why focus on page migration? Comparison with memory mode?}} We focus on page-migration  because it is OS-controlled and does not require CPU-side modifications. While we didn't compare due to the current CXL platform's lack of memory mode support,  HeMem~\cite{raybuck2021hemem} has demonstrated that page migration is superior to DRAM cache in Optane systems, as cache conflicts in memory mode result in significant overhead.

\noindent$\bullet$ \emph{\textbf{Why not exploit the MMU? Why add a dedicated core for profiling?}}  Our baselines, PTE-scan and hint-fault, do leverage the MMU (specifically, the TLB in MMU) for profiling. However, as demonstrated in Sec.\ref{sec:memory_profiling}/ Sec.\ref{sec:eval}, these approaches are hindered by high overhead and low accuracy. In contrast, our proposed NeoProf co-processor significantly enhances system performance while adding only a minimal hardware cost to device-side controllers, without any CPU-side modifications.


\noindent$\bullet$ \emph{\textbf{Why not leverage workload characteristics? Limited workload suite?}} NeoMem is general-purposed and only requires the workloads to have data locality. The exploration of more specific characteristics is beyond our scope. We chose the seven workloads for their memory-intensive nature and wide usage in previous studies. We have also included DeathstarBench in Sec.\ref{sec:eval}, a representative data-center benchmark.

\noindent$\bullet$ \emph{\textbf{The key distinction between PTE-scan and hint-fault.}} More explanations about main differences added in Sec.\ref{sec:memory_profiling}. 


\noindent$\bullet$ \emph{\textbf{Add a table of parameters.}} Added in Sec~\ref{sec:implementation}. 

\noindent$\bullet$ \emph{\textbf{More related work and per-workload analysis.}} Please refer to revision points \bthree~and \bfour. 

% \vspace{4pt}

\noindent\textbf{To review E:}

% \noindent$\bullet$ \emph{\textbf{More in-depth descriptions of the competing alternatives.}}

% Thank you for your suggestion. Please see xxx.

\noindent$\bullet$ \emph{\textbf{Will PEBS affect the utilization of NeoProf?}} NeoProf is orthogonal to PEBS. They can work together. 

\noindent$\bullet$ \emph{\textbf{The simplistic bandwidth utilization calculation?}}  In our calculations, ``read" and ``write" denote data transfer cycles, not command transfers, which already considers variable sizes (e.g., 64B or 256B).  We've refined this explanation in Sec.\ref{sec:policy}. 

 \noindent$\bullet$ \emph{\textbf{The explanation of performance improvement on GUPS.}} 
 % While the original GUPS  is random, in this work we adopt HeMem's version~\cite{raybuck2021hemem} in which some memory access regions are hotter. We have  highlighted this difference in
 We use a modified version of GUPS with hot regions.
 Please refer to Sec.~\ref{sec:exp_setup} (The Benchmarks paragraph) for details.
\clearpage
